Learning by Aligning Videos in Time

We present a self-supervised approach for learning video representations using temporal video alignment as a pretext task, while exploiting both frame-level and video-level information. We leverage a novel combination of temporal alignment loss and temporal regularization terms, which can be used as supervision signals for training an encoder network. Specifically, the temporal alignment loss (i.e., Soft-DTW) aims for the minimum cost for temporally aligning videos in the embedding space. However, optimizing solely for this term leads to trivial solutions, particularly, one where all frames get mapped to a small cluster in the embedding space. To overcome this problem, we propose a temporal regularization term (i.e., Contrastive-IDM) which encourages different frames to be mapped to different points in the embedding space. Extensive evaluations on various tasks, including action phase classification, action phase progression, and fine-grained frame retrieval, on three datasets, namely Pouring, Penn Action, and IKEA ASM, show superior performance of our approach over state-of-the-art methods for self-supervised representation learning from videos. In addition, our method provides significant performance gain where labeled data is lacking. Our code and labels are available on our research website: https://retrocausal.ai/research/

==> Tables/PennAction_Labels.tex <==
\begin{table*}
\vspace{-0.15cm}
\begin{minipage}[b]{1.0\linewidth}
\centering

{%
\begin{footnotesize}
\begin{tabular}{c|c|l|c|c}

\specialrule{1pt}{1pt}{1pt}
%\hhline{|=|=|=|}
\textbf{Action} & \textbf{Number of Phases}  & \textbf{Key Events} & \textbf{Train Set size} & \textbf{Val Set size} \\
% 
\midrule

Baseball Pitch & 4 & Knee fully up, Arm fully stretched out, Ball release & 103 & 63
\\

Baseball Swing & 3 & Start swinging bat, Bat hits the ball & 113 & 57
\\

Bench Press & 2 & Bar fully down & 69 & 71
\\

Bowling & 3 & Ball Swung back fully, Ball release & 134 & 85
\\

Clean and Jerk & 6 & Bar at hips, Fully squatting, Standing, Begin Thrusting, Beginning Balance & 40 & 42
\\

Golf Swing & 3 & Stick swung fully back, Stick hits ball & 87 & 77
\\

Jumping Jacks & 4 & Hands at shoulder (going up), Hands above head, Hands at shoulders (going down) & 56 & 56
\\

Pullups & 2 & Chin above bar & 98 & 101
\\

Pushups & 2 & Head at floor & 102 & 106
\\

Situps & 2 & Abs fully crunched & 50 & 50
\\

\specialrule{1pt}{1pt}{1pt}
\end{tabular}
\end{footnotesize}
}

\caption{Penn-Action Dataset}
\label{tab:penn_action_data}
\vspace{-0.15cm}
\end{minipage}

\end{table*}
